A Survey and Annotated Bibliography of Workflow Scheduling in Computing Infrastructures: Community, Keyword, and Article Reviews -- Extended Technical Report

Workflows are prevalent in today's computing infrastructures. The workflow model support various different domains, from machine learning to finance and from astronomy to chemistry. Different Quality-of-Service (QoS) requirements and other desires of both users and providers makes workflow scheduling a tough problem, especially since resource providers need to be as efficient as possible with their resources to be competitive. To a newcomer or even an experienced researcher, sifting through the vast amount of articles can be a daunting task. Questions regarding the difference techniques, policies, emerging areas, and opportunities arise. Surveys are an excellent way to cover these questions, yet surveys rarely publish their tools and data on which it is based. Moreover, the communities that are behind these articles are rarely studied. We attempt to address these shortcomings in this work. We focus on four areas within workflow scheduling: 1) the workflow formalism, 2) workflow allocation, 3) resource provisioning, and 4) applications and services. Each part features one or more taxonomies, a view of the community, important and emerging keywords, and directions for future work. We introduce and make open-source an instrument we used to combine and store article meta-data. Using this meta-data, we 1) obtain important keywords overall and per year, per community, 2) identify keywords growing in importance, 3) get insight into the structure and relations within each community, and 4) perform a systematic literature survey per part to validate and complement our taxonomies.

==> forest_setup.tex <==
\tikzset{
	my rounded corners/.append style={rounded corners=2pt},
}

\forestset{
	vtaxonomy/.style={
		for tree={
			grow=south,draw,minimum width=2em,
			l+=.5cm, s sep=.5cm, %
			parent anchor=south, child anchor=north,
			edge path={
	\noexpand\path[line width=1pt,\forestoption{edge}]
	(\forestOve{\forestove{@parent}}{name}.parent anchor) -- +(0,-10pt) -|   
	(\forestove{name}.child anchor)\forestoption{edge label};
			}
		},
	},
}

\forestset{
	htaxonomy/.style={
		for tree={
			grow=east,draw,minimum width=3em,
			l+=.5cm, s sep=1cm,
			parent anchor=east, child anchor=west,
			edge path={
				\noexpand\path[line width=1pt,\forestoption{edge}]
				(\forestOve{\forestove{@parent}}{name}.parent anchor) -- +(10pt,0) |-   
				(\forestove{name}.child anchor)\forestoption{edge label};
			}
		}
	},
}

==> scheduling_systems.tex <==
\section{Workflow Execution Systems}
\label{workflow-execution-systems}

\todo[inline]{Remove this section, as this would fit a survey version of the SC article better?}

During the past decades, several workflow execution systems have been proposed by both industry and academia.
Andreadis et al. \add{cite SC18 work} introduce a novel reference architecture for workflow execution systems.
In this section we provide an overview of several well-known workflow execution systems.


\add{Record for each scheduler te complete set of documents used to analyze the scheduler.}

\subsection{Overview}

In this section we provide an overview of several workflow execution systems.
In table \todo{add table} we highlight the optimization target, scheduling technique and scheduler structure used.


List of workflow management systems:


\tablehead{\toprule Name & \makecell[l]{Optimization\\goal} & \makecell[l]{Scheduling\\technique} & \makecell[l]{Scheduler\\structure} \\
\midrule}
\tabletail{\bottomrule}

	\begin{supertabular}{llll}
		Amadeus & ? & ? & ? \\
		ICENI & ? & ? & ? \\
		ASKALON & ? & ? & ? \\
		Pegasus & ? & ? & ? \\
		Taverna & ? & ? & ? \\
		Kepler & ? & ? & ? \\
		Triana & ? & ? & ? \\
		Hadoop & ? & ? & ? \\
		Dryad & ? & ? & ? \\
		Borg & ? & ? & ? \\
		Kubernetes & ? & ? & ? \\
		Graphene & ? & ? & ? \\
		Flowmanager & ? & ? & ? \\
		Firmament & ? & ? & ? \\
		TITAN & ? & ? & ? \\
		Arvados   & ? & ? & ? \\
		Taverna   & ? & ? & ? \\
		Galaxy   & ? & ? & ? \\
		SHIWA   & ? & ? & ? \\
		Oozie   & ? & ? & ? \\
		DNANexus   & ? & ? & ? \\
		BioDT   & ? & ? & ? \\
		Agave   & ? & ? & ? \\
		DiscoveryEnvironment   & ? & ? & ? \\
		Wings   & ? & ? & ? \\
		Knime   & ? & ? & ? \\
		Snakemake   & ? & ? & ? \\
		BPipe   & ? & ? & ? \\
		Ruffus   & ? & ? & ? \\
		NextFlow   & ? & ? & ? \\
		Luigi   & ? & ? & ? \\
		SciLuigi.  & ? & ? & ? \\
		\makecell[l]{Luigi Analysis\\ Workflow (LAW)}   & ? & ? & ? \\
		GATK Queue   & ? & ? & ? \\
		Yabi   & ? & ? & ? \\
		Ketrew   & ? & ? & ? \\
		Pegasus   & ? & ? & ? \\
		Airflow   & ? & ? & ? \\
		Cosmos   & ? & ? & ? \\
		Pinball   & ? & ? & ? \\
		bcbio   & ? & ? & ? \\
		Chronos   & ? & ? & ? \\
		Azkaban   & ? & ? & ? \\
		Apache NiFi   & ? & ? & ? \\
		flowr (R-based)   & ? & ? & ? \\
		Mistral   & ? & ? & ? \\
		nipype   & ? & ? & ? \\
		End of Day   & ? & ? & ? \\
		BioDSL   & ? & ? & ? \\
		BigDataScript   & ? & ? & ? \\
		Omics Pipe   & ? & ? & ? \\
		Ensembl Hive   & ? & ? & ? \\
		QuickNGS   & ? & ? & ? \\
		GenePattern   & ? & ? & ? \\
		Chipster   & ? & ? & ? \\
		\makecell[l]{The Genome \\Modeling System} & ? & ? & ? \\
		Cuneiform   & ? & ? & ? \\
		Anvaya   & ? & ? & ? \\
		Makeflow   & ? & ? & ? \\
		Airavata   & ? & ? & ? \\
		Pyflow   & ? & ? & ? \\
		Cluster Flow   & ? & ? & ? \\
		Unipro UGENE   & ? & ? & ? \\
		CloudSlang   & ? & ? & ? \\
		Stacks   & ? & ? & ? \\
		Leaf   & ? & ? & ? \\
		omictools   & ? & ? & ? \\
		JDL & ? & ? & ? \\
		YAWL   & ? & ? & ? \\
		Triquetrum   & ? & ? & ? \\
		Kronos   & ? & ? & ? \\
		qsubsec   & ? & ? & ? \\
		YesWorkflow   & ? & ? & ? \\
		GWF   & ? & ? & ? \\
		Fireworks.   & ? & ? & ? \\
		NGLess   & ? & ? & ? \\
		pypipegraph   & ? & ? & ? \\
		Cromwell   & ? & ? & ? \\
		Dagobah & ? & ? & ? \\
		sushi   & ? & ? & ? \\
		\makecell[l]{Clinical Trial \\Processor} & ? & ? & ? \\
		Noodles   & ? & ? & ? \\
		Swift   & ? & ? & ? \\
		Consonance   & ? & ? & ? \\
		Dog   & ? & ? & ? \\
		Produce   & ? & ? & ? \\
		LONI Pipeline   & ? & ? & ? \\
		Cpipe   & ? & ? & ? \\
		AWE   & ? & ? & ? \\
		(Py)COMPSs   & ? & ? & ? \\
		KLIKO   & ? & ? & ? \\
		Script of Scripts   & ? & ? & ? \\
		XNAT  & ? & ? & ? \\
		Metapipe   & ? & ? & ? \\
		OCCAM   & ? & ? & ? \\
		Copernicus   & ? & ? & ? \\
		iRODS   & ? & ? & ? \\
		VisTrails   & ? & ? & ? \\
		Bionode Watermill   & ? & ? & ? \\
		BIOVIA & ? & ? & ? \\
		Dagman & ? & ? & ? \\
		UNICORE   & ? & ? & ? \\
		Toil  & ? & ? & ? \\
		Cylc   & ? & ? & ? \\
		\makecell[l]{Autodesk Cloud \\Compute Canon}   & ? & ? & ? \\
		Civet   & ? & ? & ? \\
		Cumulus   & ? & ? & ? \\
		HIVE  & ? & ? & ? \\
		Cloudgene   & ? & ? & ? \\
		FASTR   & ? & ? & ? \\
		BioMake   & ? & ? & ? \\
		remake   & ? & ? & ? \\
		SciFloware   & ? & ? & ? \\
		OpenAlea   & ? & ? & ? \\
		COMBUSTI/O   & ? & ? & ? \\
		BioCloud   & ? & ? & ? \\
		Triana   & ? & ? & ? \\
		Kepler   & ? & ? & ? \\
		Anduril   & ? & ? & ? \\
		dgsh   & ? & ? & ? \\
		EDGE bioinformatics   & ? & ? & ? \\
		Pachyderm   & ? & ? & ? \\
		Digdag   & ? & ? & ? \\
		Agua & ? & ? & ? \\
		\makecell[l]{BioDepot Workflow\\ Builder (BwB)}   & ? & ? & ? \\
		IMP & ? & ? & ? \\
		Butler   & ? & ? & ? \\
		adage / yadage   & ? & ? & ? \\
		HI-WAY & ? & ? & ? \\
		OpenMOLE   & ? & ? & ? \\
		Biopet   & ? & ? & ? \\
		Nephele   & ? & ? & ? \\
		TOPPAS   & ? & ? & ? \\
		SBpipe   & ? & ? & ? \\
		Dray   & ? & ? & ? \\
		GenomeVIP   & ? & ? & ? \\
		GridSAM   & ? & ? & ? \\
		Roddy   & ? & ? & ? \\
		SciFlo  & ? & ? & ? \\
		GNU Guix  & ? & ? & ? \\
		Porcupine   & ? & ? & ? \\
		Parsl & ? & ? & ? \\
		ECFLOW  & ? & ? & ? \\
		Ophidia   & ? & ? & ? \\
		WebLicht   & ? & ? & ? \\
		GATE Cloud   & ? & ? & ? \\
		SCIPION   & ? & ? & ? \\
		Ergatis   & ? & ? & ? \\
		TIGR "Workflow"   & ? & ? & ? \\
		Archivematica   & ? & ? & ? \\
		Martian   & ? & ? & ? \\
		BioMAJ   & ? & ? & ? \\
		Conveyor   & ? & ? & ? \\
		Biopipe   & ? & ? & ? \\
		Wildfire   & ? & ? & ? \\
		BioWBI   & ? & ? & ? \\
		BioWMS   & ? & ? & ? \\
		BioMoby   & ? & ? & ? \\
		SIBIOS   & ? & ? & ? \\
		NGSANE   & ? & ? & ? \\
		Pwrake   & ? & ? & ? \\
		Nesoni   & ? & ? & ? \\
		Skam   & ? & ? & ? \\
		TREVA   & ? & ? & ? \\
		EGene   & ? & ? & ? \\
		WEP   & ? & ? & ? \\
		Microbase   & ? & ? & ? \\
		e-Science Central   & ? & ? & ? \\
		Cyrille2   & ? & ? & ? \\
		PaPy   & ? & ? & ? \\
		JobCenter   & ? & ? & ? \\
		CoreFlow   & ? & ? & ? \\
		dynamic-pipeline   & ? & ? & ? \\
		XiP   & ? & ? & ? \\
		Eoulsan   & ? & ? & ? \\
		CloudDOE   & ? & ? & ? \\
		BioPig   & ? & ? & ? \\
		SeqPig   & ? & ? & ? \\
		zymake   & ? & ? & ? \\
		JMS   & ? & ? & ? \\
		\makecell[l]{CLC Genomics \\Workbench}   & ? & ? & ? \\
		NG6   & ? & ? & ? \\
		VIBE   & ? & ? & ? \\
		WDL & ? & ? & ? \\
		SciFlow   & ? & ? & ? \\
		Bioshake   & ? & ? & ? \\
		SciPipe   & ? & ? & ? \\
		Kapacitor / TICKscripts   & ? & ? & ? \\
		AiiDA & ? & ? & ? \\
		Reflow & ? & ? & ? \\
		Resolwe & ? & ? & ? \\
		Yahoo! Pipes & ? & ? & ? \\
		Walrus   & ? & ? & ? \\
		Apache Beam   & ? & ? & ? \\
		CLOSHA   & ? & ? & ? \\
		WopMars   & ? & ? & ? \\
		flowing-clj   & ? & ? & ? \\
		Plumbing and Graph   & ? & ? & ? \\
		LabView   & ? & ? & ? \\
		MyOpenLab   & ? & ? & ? \\
		Max/MSP   & ? & ? & ? \\
		NoFlo   & ? & ? & ? \\
		Flowstone   & ? & ? & ? \\
		HyperLoom   & ? & ? & ? \\
		Dask   & ? & ? & ? \\
		Stimela   & ? & ? & ? \\
		JTracker   & ? & ? & ? \\
		PipelineDog   & ? & ? & ? \\
		DALiuGE   & ? & ? & ? \\
		Overseer   & ? & ? & ? \\
		Squonk   & ? & ? & ? \\
		GC3Pie   & ? & ? & ? \\
		Fractalide   & ? & ? & ? \\
		TOGGLe   & ? & ? & ? \\
		Askalon   & ? & ? & ? \\
		Eclipse ICE  & ? & ? & ? \\
		SAW   & ? & ? & ? \\
		dispel4py   & ? & ? & ? \\
		Jobber   & ? & ? & ? \\
		NeatSeq-Flow   & ? & ? & ? \\
		S4M   & ? & ? & ? \\
		Loom   & ? & ? & ? \\
		Watchdog   & ? & ? & ? \\
		phpflo   & ? & ? & ? \\
		BASTet & ? & ? & ? \\
		Tavaxy & ? & ? & ? \\
		Ginflow & ? & ? & ? \\
		SciApps  & ? & ? & ? \\
		Stoa & ? & ? & ? \\
		CK Framework   & ? & ? & ? \\
		QosCosGrid (QCG)   & ? & ? & ? \\
	\end{supertabular}

\todo[inline]{make table highlighting per system: name (A/I), optimization target, scheduling technique, scheduler structure ((de)central/hybrid)}

==> taxonomy_forest.tex <==
\begin{figure*}
\begin{adjustbox}{width=\linewidth}
\begin{forest}
      for tree={
        line width=1pt,
        if={level()<2}{
          my rounded corners,
          draw=linecol,
        }{},
        edge={color=linecol, >={Triangle[]}, ->},
        if level=0{%
          l sep+=0.5cm,
          align=center,
          parent anchor=south,
        }{%
          if level=1{%
            parent anchor=south west,
            child anchor=north,
            tier=parting ways,
            align=center,
            font=\bfseries,
            for descendants={
              child anchor=west,
              parent anchor=west,
              anchor=west,
              align=left,
            },
          }{
            if level=2{
              shape=coordinate,
              no edge,
              grow'=0,
              calign with current edge,
              xshift=20pt,
              for descendants={
                parent anchor=south west,
                l sep+=-20pt
              },
              for children={
                edge path={
                  \noexpand\path[\forestoption{edge}] (!to tier=parting ways.parent anchor) |- (.child anchor)\forestoption{edge label};
                },
                font=\bfseries,
                for descendants={
                  no edge,
                },
              },
            }{},
          },
        }%
      },
      [Workflow Scheduling
        [(Optimization) Target
          [
            [Security \& Privacy]
            [Elasticity]
            [Fault tolerance]
            [Makespan]
            [Priority]
            [Fairness]
            [Resource utilization]
            [Data locality]
            [Runtime]
            [Cost]
          ]
        ]
        [Optimization strategy
	        [
		        [Constraint
			        [Global\\
			        Local]
		        ]
		        [Focus
			        [Multi-criteria\\
			        Single criterion]
		        ]
	        ]
        ]
        [Workflow Formalism
          [
            [Bag-of-task]
            [\acrshort{dag}]
            [\acrshort{bpmn}]
            [\acrshort{pn}]
            [\acrshort{yawl}]
            [\acrshort{cwl}]
          ]
        ]
        [Scheduling Technique
          [
            [Heuristics
	          [Greedy\\
	          Simulated Annealing\\
	          Ant Colony Optimization\\
	          Iterative Ordinal Optimization]
            ]
            [Meta-heuristic]
            [Genetic Algorithm]
            [Neural Network]
            [Exhaustive Search]
            [Game Theory]
            [Random]
          ]
        ]
        [Scheduler structure
	        [
		        [Centralized]
		        [Decentralized]
		        [Hierarchical]
	        ]
	    ]
	    [Resource type
		    [
			    [None]
			    [Container]
			    [VM]
			    [Thread]
			    [Core]
			    [CPU]
			    [Machine]
			    [Cluster]
		    ]
	    ]
        [Scheduling Scheme
          [
            [Static
              [User-directed\\
              Simulation-based]
            ]
            [Dynamic
              [Prediction-based\\
              Just-in-time\\
              Run-time
              ]
            ]
          ]
        ]
      ]
\end{forest}
\end{adjustbox}
\caption{General workflow scheduler taxonomy. Maximum depth of four visible.} 
\label{fig:scheduling_approaches}
\end{figure*}

==> terminology.tex <==
\section{Terminology}
\todo[inline]{Most likely: Delete this section}

This section provides an overview of terms commonly used by the community, are rather unfamiliar due to being emerging, or are mentioned to avoid ambiguity and confusion.

\begin{description}
	\item[A task] is a small unit of work, e.g. a piece of code or program that is self-contained.
	\item[A workflow] is a set of tasks with their data or computational dependencies explicitly described. Applications are often modeled this way.
	\item[An entry task] of a workflow is a task that does not have any incoming dependencies and thus, can be started immediately.
	\item[An exit task] of a workflow is a task that does not have any outgoing dependencies.
	\item[The critical path] of a workflow is the maximum time from any entry task to any exit task. It represents the minimal time required to execute a workflow provided infinite resources (no bottleneck).
	\item[Serverless] is an emerging paradigm where consumers do not manage any infrastructure i.e., servers, themselves. All infrastructure is managed and operated by the cloud provider.
	\item[A scheduler] manages both the resources and incoming jobs in a datacenter. It can acquire resources on behalf of the customer and decides the order of tasks and where they will be executed.
	\item[The allocation policy] is the algorithm that computes task placement. This policy often includes multiple parameters to optimize towards a certain target.
	\item[The provisioning policy] is the algorithm used to compute how many resources should be released or acquired.
	\item[An autoscaler] is a component that automatically scales up and down resources on behalf of the customer according to the provisioning policy and (past) state information about the system.
	\item[A schedule] is the \enquote{plan} devised by the scheduler. The schedule dictates the order in which the tasks will be placed and on which resources. These decisions are based on the allocation and provisioning policies.
	\item[An offline] scheduler computes the entire schedule before starting to execute any task, and thus strictly adheres to the computed schedule.
	\item[An online] scheduler computes a schedule dynamically. If workflows enter the system during runtime, the schedule gets updated according to the used policies.
	\item[Edge computing] is an emerging paradigm where mini-datacenters are put closer to customers. They contain less resources than full datacenters -- which are sparsely spread around the world -- yet offer lower latency due to their geographical proximity.
	\item[A \gls{nfr}] is a requirement that specifies not \textit{how} a system must perform a certain operation, but a requirement that should or must be fulfilled. An example of a \gls{nfr} is a deadline.
	\item[The makespan] of a workflow is the time elapsed be the start of the first task and the end of the last task.
\end{description}

==> workflow_execution_model.tex <==
\section{Generic workflow processing model}
\label{sct:generic_workflow_processing_model}

\add{Text about the generic workflow model as discussed with Alex.}
